Decomposition of Nonlinear Dynamical Systems Using Koopman Gramians

In this paper we propose a new Koopman operator approach to the decomposition of nonlinear dynamical systems using Koopman Gramians. We introduce the notion of an input-Koopman operator, and show how input-Koopman operators can be used to cast a nonlinear system into the classical state-space form, and identify conditions under which input and state observable functions are well separated. We then extend an existing method of dynamic mode decomposition for learning Koopman operators from data known as deep dynamic mode decomposition to systems with controls or disturbances. We illustrate the accuracy of the method in learning an input-state separable Koopman operator for an example system, even when the underlying system exhibits mixed state-input terms. We next introduce a nonlinear decomposition algorithm, based on Koopman Gramians, that maximizes internal subsystem observability and disturbance rejection from unwanted noise from other subsystems. We derive a relaxation based on Koopman Gramians and multi-way partitioning for the resulting NP-hard decomposition problem. We lastly illustrate the proposed algorithm with the swing dynamics for an IEEE 39-bus system.

==> ACC 2018-Koopman Decomposition/Section/conclusion.tex <==
\section{conclusion}

==> ACC 2018-Koopman Decomposition/Section/experiment.tex <==
\section{experiment}

==> ACC 2018-Koopman Decomposition/Section/introduction.tex <==
\section{Introduction}
The design and control of complex systems is usually broken down into simpler modules, e.g. different geographically dispersed subsystems such as different balancing authority areas in power networks and various vertically integrated functionalities such as routing and congestion control in communication networks. Despite modular design being a common practice, the decomposition of the system into different modules is often based on engineering intuition rather than principled methodologies. 

%In this paper we study the problem of model decomposition for nonlinear systems, for the purpose of distributed control design.  Distributed control design has become increasingly important with the advent of interdependent large-scale infrastructure systems, smart cities, design of network architectures, and coordination and control problems for large fleets of independent agents.   The combination of scale and dynamical complexity of these systems makes it computationally difficult to design global control solutions.  

%Design of distributed control architectures can be roughly described as a three step process.  First, the system is decomposed into subsystems, second, distributed controllers are designed to stabilize individual subsystems, and third, the overall interconnected system is assessed for global stability.  The first step of this process is critical, and is the focus of this paper, since a poor system or model decomposition can affect all subsequent steps of distributed control design.    

For example, in some applications, the physical layout or construction of a system dictates the subsystem structure.  For example, in multi-cellular biological systems, the subsystems are a natural consequence of physical separation by the membrane barrier \cite{regot2011distributed, tamsir2011robust,miller2001quorum}.  In critical infrastructure systems, e.g. the power grid or water distribution systems, the subsystem structure is traditionally defined based on distance and connectivity of buses, nodes or junctions \cite{chiang2016large,li2008interdependency}.  However, this choice of decomposition is critical since a poor system or model decomposition can introduce fundamental limits into distributed controller performance. 


Moreover, there are many scenarios where a suitable system decomposition may not be known {\it a priori}, e.g. design of large-scale or ad-hoc communication networks \cite{chiang2016fog, chiang2007layering, chiang2016large} or cyber-physical systems made of agile teams of agents.  In such situations, the system decomposition must be identified, using appropriate criteria that enable performance of a distributed controller.  This is especially true of extremely large scale networks involving thousands of variables where synthesis of a global controller may not be computationally feasible.   

There are many existing methods for model decomposition \cite{sanchez2014hierarchical,raak2014partitioning,chiang2007layering};   each method decomposes systems based on different properties.  Sanchez-Garcia et al. \cite{sanchez2014hierarchical} decomposes a system into subsystems by examining the spectrum of a matrix encoding connectivity in power networks.  When that matrix is the admittance matrix, the decomposition reflects static connectivity structure; when the matrix is power flow, the decomposition reveals islands with minimal power flow disruption.  Chiang, Low, and Doyle showed that system decomposition for layered network design problems can be thought of as vertical and horizontal decomposition of optimization problems with utility functions corresponding to different Quality of Service metrics, e.g. fairness, minimal congestion, or efficiency \cite{chiang2007layering}.   Raak et al. \cite{raak2014partitioning} use the Koopman operator to define a lifted linear representation of an open-loop nonlinear system.  They introduce a decomposition method based on the point-spectrum of the Koopman operator.   

In this paper we adopt a similar Koopman operator approach for system decomposition as Raak et al. \cite{raak2014partitioning}, but derive the decomposition from input-output properties directly computed from Koopman Gramians \cite{YeungGramians}.  Koopman operators are especially powerful, since they allow us to transform nonlinear analysis and control problems into linear problems.  Furthermore, system identification methods for Koopman operators have made it possible to perform analysis and control design in a purely data-driven fashion \cite{mezic2004comparison,mezic2005spectral,rowley2009spectral,williams2015data}.  Such an approach is especially valuable in data-driven control and analysis problems, e.g., Internet of Things applications \cite{chiang2016fog}, intelligent load control problems in infrastructure systems \cite{trudnowski2006power}, or design of multicellular biocircuits \cite{tamsir2011robust}.  
%We use Koopman operators to perform gramian based decompositions on the system.  Gramians encode properties of input-output dynamics; partitioning system states based on the grammian results in computational certificates of bounded input-bounded output (or state, with full state outputs) stability. Koopman grammians can be computed directly from time-series data or learned directly from a nonlinear system model, which provides flexibility depending on the application setting.    

Specifically, we introduce the notion of an input-Koopman operator, show how input-Koopman operators can be used to cast a nonlinear system into the classical state-space form, and identify conditions under which input and state observable functions are well separated.  We then extend an existing method of dynamic mode decomposition for learning Koopman operators from data known as deep dynamic mode decomposition to systems with controls or disturbances.  We illustrate the accuracy of the method in learning an input-state separable Koopman operator for an example system, even when the underlying system exhibits mixed state-input terms.  We next introduce a nonlinear decomposition algorithm, based on Koopman Gramians, that maximizes internal subsystem observability and disturbance rejection from unwanted noise from other subsystems.  As the resulting decomposition problem is NP-hard, we derive a relaxation based on Koopman Gramians and multi-way partitioning.  We illustrate the proposed algorithm with the swing dynamics for am IEEE 39-bus system        

The rest of the paper is organized as follows.  Section II introduces input-Koopman operators and reviews the theory of input-Koopman operators.  Section III discusses several results and techniques for learning Koopman operators and the associated Koopman Gramians.  Section IV presents the proposed Koopman decomposition algorithm, and Section V illustrates its application on an IEEE 39-bus system.  


%Data driven 
%Nonlinear 
%Input-Output, multiple perspectives at play. 




==> ACC 2018-Koopman Decomposition/Section/reduction.tex <==
\section{Model reduction}

==> ACC 2018-Koopman Decomposition/Section/system.tex <==
\section{Model Decomposition}
We consider a class of nonlinear systems which have affine control perturbations \textcolor{red}{Cite all of the Isidori and Kotkotovic people}.  Namely we write the system as 
\begin{equation}\label{eq:nonlinear_affine_system}
\begin{aligned}
\dot{x} &= f(x) + g(u)  \\ 
y &= h(x)
\end{aligned}
\end{equation}
where $f,g,h  \in \mathbb{R}^n$ is assumed to be continuously differentiable functions (with $f,g \in C^p\left[0,\infty\right)$ where $p \geq 2$) with respect to $x,u,$ and $t$, respectively.   Without loss of generality, we suppose that $u = 0$ implies that $g(u) = 0$, i.e. any zeroth-order terms in a Taylor expansion of $g(u)$ are subsumed into the definition of $f(x)$. 
\textcolor{red}{Explain for the layman why this is not a loss of generality. Use the Taylor series argument on C-differentiable functions. }

We suppose that $f,g$ and $h$ are time-invariant, i.e. they are directly dependent on $t$.  We model the state $x(t) \in \mathbb{R}^n$ and the input $u(t) \in\mathbb{R}^m$ for all $t \in \left[0,\infty\right).$ 

In this paper, we restrict our attention to nonlinear models that can expressed with an actuated Koopman equation of the form 
\begin{equation}
\dot{\psi}_x(x) = K_x \psi_x(x) + K_u \psi_u(u) 
\end{equation}
    
The Koopman grammian was introduced in \cite{Grammian2017}    
as a way to quantify the controllability and observability of a nonlinear dynamical system.  Here we investigate using the Koopman grammian to obtain a decomposition of the nonlinear system with BIBO stability certificates. 

In our problem, we suppose there are two objectives.  First, we suppose that we want to maximize controllability and observability with respect to a series of input and output channels that represent a system operator's perspective. \textcolor{red}{ Add more writing to clarify what perspectives mean intuitively, motivate blah blah}.  Second, we suppose we want to minimize controllability and observability with respect to a outsider's perspective. 

We model the perturbed system with the form 
\begin{equation}\label{eq:SO_system}
\begin{aligned}
\dot{x} &= f(x) + g(u_S,u_E) \\ &= f(x) + g_S(u_S) + g_E(u_E)  \\ 
y_S &= h_S(x)\\ 
y_E & = h_E(x)  
\end{aligned}
\end{equation}
We suppose, as in \ref{Kutz2015,Williams2016} that an equivalent actuated Koopman system exists for the system (\ref{eq:nonlinear_affine_system}).  
In the presence of two input channels $u_S$ and $u_E$, the question arises as to what the structure of the Koopman system will be.   The following lemma clarifies the system structure. 

\begin{lemma}
Consider system (\ref{eq:nonlinear_affine_system}).  The control Koopman equation for this system is given as 
\begin{equation}
\dot{\psi}(x) = K_x\psi(x)) + K_u\psi_u(u)  
\end{equation}
\end{lemma}
\begin{proof}
More generically, we note that system (\ref{eq:nonlinear_affine_system}), is a special instance of the form of systems studied in \cite{Kutz2015}.  Thus, there exists a control Koopman operator that satisfies the control-Koopman equation
\begin{equation}
\dot{\psi} (x) = K\psi(x,u) 
\end{equation}
Now for our class of nonlinear affine control systems, we know that the Koopman equation can be written \cite{Rowley2015} 
\begin{equation}
\begin{aligned}
\dot{\psi}(x) &= \frac{\partial \psi(x) }{\partial x} \left( f(x) + g(u) \right) \\&=   K\psi(x,u) = K_x \psi_x(x) + K_u \psi_u(u) + K_{xu} \psi_{xu}(x,u)  
\end{aligned}
\end{equation}
where in the last equation we have partitioned $\psi(x,u)$ into terms that directly depend on $x$, $u$, or a mix of the two terms.  Such a partition is always possible, even if one of the terms is trivial.  It suffices to show that the cross-term doesn't exist.  To see this, we take second order partials 

\begin{equation}
\begin{aligned}
 \frac{\partial^2}{\partial u\partial x}\dot{\psi}(x) & =  \frac{\partial^2}{\partial u\partial x} \left(\frac{\partial \psi(x) }{\partial x} \left( f(x) + g(u) \right) \right)\\ &= \frac{\partial^3 \psi(x) }{\partial u \partial^2 x} \left(f(x) + g(u) \right)    \\ & \hspace {3mm} +  \frac{\partial \psi(x) }{\partial x}\frac{\partial}{\partial u}\frac{\partial}{\partial x}\left(f(x) + g(u)\right)\\
 & = 0 
\end{aligned}
\end{equation}
The first term vanishes due to the strict independence of $\psi(x)$ with respect to $u$. 
The second term vanishes due to the affine separation between dependencies of $x$ and $u$ in $f(x)$ and $g(u).$  

In the Koopman equation, taking second order partials results in 
\begin{equation}
\begin{aligned}
\frac{\partial^2}{\partial u\partial x} K\psi(x,u) &=  \frac{\partial^2}{\partial u\partial x} K_x \psi_x(x) + K_u \psi_u(u) + K_{xu} \psi_{xu}(x,u)\\ 
&= 0 + 0 + \frac{\partial^2}{\partial u\partial x} K_{xu} \psi_{xu}(x,u) 
\end{aligned}
\end{equation}
which implies that 
\begin{equation}
\frac{\partial^2}{\partial u\partial x} K_{xu} \psi_{xu}(x,u) = 0 
\end{equation}
By convention, all constant Koopman basis terms are kept in $\psi_x(x)$, which implies that $\psi_{xu}$ has no constant terms, only terms that depend both $x$ and $u$.  The implication of the above equation is that $\psi_{xu}(x,u)$ has only zero and first order terms.  However, since all zero order terms are already in $\psi_x(x)$ and first order terms do not involve mixtures of $x$ and $u$, $\psi_{xu}(x,u) \equiv 0$ for all $x$ and $u.$ 
\end{proof}
This lemma suggests that the system structure of a Koopman operator reflects the dependency structure of the underlying  nonlinear affine system from which it is derived.    In proving this, we have identified a class of nonlinear affine systems that lend themselves to Koopman analysis, and by extension, the classical analysis techniques of control theory for linear time-invariant systems.   However, the Koopman system may be infinite-dimensional.  Whenever the system satisfies Carleman closure \cite{}, then the system is said to have a finite-dimensional Koopman representation.  Otherwise, the  matrices may be infinite-dimensional and require a finite-dimensional approximation. 

We now consider the Koopman system model for a system with external and operator control channels.  The following lemma shows that the structure of the Koopman model mirrors the input structure of system \ref{eq:SO_system}
\begin{lemma}

\end{lemma}


The next lemma is a direct extension of Lemma \ref{lemma:affine_Koopman_partition}

We suppose that an actuated-Koopman equation can be computed for each system model.  We remark that $f(x)$ defines the core dynamics of the system; thus the Koopman operator ${\cal K}_x$ defined with respect to $f$ is the same for both systems, while the Koopman control operator ${\cal K}_u$ and Koopman output equation may be different for each system. 
\begin{lemma}
Given the system (\ref{eq:SO_system}), the Koopman actuated-equations for system operator are of the form 
\begin{equation}
\begin{aligned}
\dot{\psi}^S_x(x) &= K_x^S \psi^S_x(x) + K^S_u \psi^S_u(u) \\
y  &= W^S \psi^S_x(x) 
\end{aligned}
\end{equation}
while the Koopman actuated-equations for the external system (\ref{eq:ES_system}) are given 
\begin{equation}
\begin{aligned}
\dot{\psi}_x^E(x) &= K_x^E \psi^E_x(x) + K^E_u \psi^E_u(u) \\
y  &= W^E \psi^E_x(x) 
\end{aligned}
\end{equation}
Moreover, $\psi^S_x(x) = \psi^S_u(x)$ and $K_x^S = K_x^E.$
\end{lemma}
\begin{proof}
First, from \cite{Kutz2016,Williams2017} \textcolor{red}{Check this reference for rigor!}, we know that a Koopman control equation can be defined for both the external and system model, since they are of the form of $\eqref{eq:nonlinear_affine_system}.$    Moreover, these equations must hold for all $x \in \mathbb{R}^n$ and $u\in\mathbb{R}^m$, including $u=0.$  By construction, $u=0$ implies $\dot{x} = f(x)$ for both systems.   Suppose $\psi^j_u(0) \neq 0$ for $j= S$ or $E$.



Considering the special case $u=0$ which implies $g(u) = 0$, the system then can be regarded as an autonomous system defined by $f(x)$. So for arbitrary $x$, the Koopman actuated equations for system operator and external system should be same. This implies that $K_x^{S} = K_{x}^{E}$.
\end{proof}

\begin{equation}
\begin{aligned}
	\psi_{x}(x_{n}) &= K_x\psi_{x}(x_{n-1}) + K_u\psi_{u}(u_{n-1}) \\
    & = K_{x}^{n}\psi_{x}(x_{0}) + \sum_{i=0}^{n} K_{x}^{i}K_{u}\psi_{u}(u_{i}).
\end{aligned}
\end{equation}
So the lifted Koopman grammian 
\begin{equation}
\begin{aligned}
X_c  &=  \sum_{i=0}^n (K_x)^i K_u K_u^* (K_x^*)^{i} \\
X_o  &= \sum_{i=0}^{n} W(K_x)^{i}(K_x^{*})^{i}W^{*}
\end{aligned}
\end{equation}

Once the models have been cast in the Koopman grammian framework, we can treat the problem as a decomposition on a single dynamical system with two linear time-invariant representations. 

The insider model:
	\begin{eqnarray}
		\dot{x} &=& Ax + B_{in}u, \\
		       y &=& C_{in}x.
	\end{eqnarray}
	And the outsider model:
	\begin{eqnarray}
	\dot{x} &=& Ax + B_{out}u, \\
	y &=& C_{out}x.
	\end{eqnarray}
	
	Generally speaking, $B_{in}, C_{in}$ is much more dense than $B_{out}, C_{out}$. When doing the decomposition for this system, we want to achieve the following property:
	for each subsystem, we want to let the insider have a minimum gramiams, in the meanwhile, outsider have the maximum gramiams. 
	\begin{eqnarray}
		&\min &\sum_{i} \|G_{in}^{i}\| \\
		&\max &\sum_{i} \|G_{out}^{i}\|
	\end{eqnarray}
	To clarify our motivation, let's first consider the following questions:
	\begin{itemize}
		\item (a) We should give the strict definition of insider and outsider ? They are totally different or overlapped ?
		\item (b) We need to give the strict definition of $G_{in}^{i}$ and $G_{out}^{i}$. This relies on clear definition of subsystem(input, output, interconnected factors), then we can compute the gramians .  
		\item (c) What is the incentive for decomposition ? Think about this, 
		assume we don't decompose the system, what should we handle this case ? Another realization ?
		\item (d) If we can do (c), \textcolor{red}{why we do the decomposition}? We should give some motivations here. 
		\item (e) After we have clarified the problems above, the core problem is how to formulate this as an optimization problem even it is NP hard. Always, the clustering problem is NP hard. Our problem is much complicated than normal clustering problem.
        \item (f) If we use Koopman Operator, how could we preserve the structure of our systems ?    
	\end{itemize}
    Also, let's look at the Fig. \ref{fig: motivation}. The left side is our original system. After we do the decomposition, we may find that, for each subsystem, we need to redefine its input, output. \textcolor{red}{So that means our result of partition determines how to compute the gramiams, while in the same time, we also want to do the partition based on gramiams}. This dilemma makes the problem more complicated.  
    \begin{figure}[ht]
    	\centering
    	\includegraphics[width = 8.5cm,height= 4.0cm]{./Figures/motivation}
    	\caption{Model Decomposition}
    	\label{fig: motivation}
    \end{figure}
	To be continued...
	
	
	Some works may be helpful to relief this problem:
	\textcolor{red}{State aggregation} \cite{ishizaki2012clustering} \cite{deng2010building}.  \cite{ishizaki2012clustering} does the  clustering based on the local controlability, however, it has a very strong constraints on the underlying systems. \cite{deng2010building} treats the system a stable Markov process, and does the state aggregation based on minimizing the difference between two Markov process. \\
	
	**********************************************
	\textcolor{red}{The following is our previous idea}.\\
	Consider a continuous time system of the form:
	\begin{eqnarray*}
		\dot{x} &=& f(x)  
	\end{eqnarray*}
    where we assume that $f \in R^{n}$ is continuously differentiable. Our goal is to make a decomposition of  states $X$ such that within each subsystem, the states are strongly infected by each other; in the meanwhile, states outside this subsystem have less influence compared to states within. \textcolor{red}{explanations why we do decomposition}. To do this, we need to solve the following challenges
    \begin{itemize}
    	\item Usually, dynamic system is nonlinear.
    	\item For clustering, how to define the link weight between two states? Also, the graph is directed and contains self-loop links. 
    \end{itemize}

	For the first challenge, our idea here is to use Koopman operator. the Koopman operator is a canonical operator which is the infinite-dimensional map describing the evolution of observables over time. Specially the Koopman operator could be expressed as 
	\begin{eqnarray*}
		\psi(\dot{y}) = \mathcal{K}\psi(y),
	\end{eqnarray*} 
where $\psi(Y)$ is usually an infinite-dimensional observable belong to the subspace of all observables $M_{\psi}$. In this paper, we assume that the original states are contained in these observables. So $Y = [x, \Phi(x)]^{T}$ and we get
	\begin{eqnarray*}
		\psi({[\dot{x}~~\dot{\Phi}(x)]^{T}}) = \mathcal{K}\psi([x~~\Phi(x)]^{T}).
	\end{eqnarray*} 
Also, we use the full state observable $\psi(y = x) = x$ and this will lead to 
\begin{eqnarray}
	\left[\begin{matrix}
		\dot{x}  \\ \dot{\Psi}(x)
	\end{matrix}\right] = \left[\begin{matrix}
		\mathcal{K}_{11} & \mathcal{K}_{12}\\
		\mathcal{K}_{21} & \mathcal{K}_{22}\\
\end{matrix}\right]	\left[\begin{matrix}
     x  \\ \Psi(x)
\end{matrix}\right].  \label{eq: 1}
\end{eqnarray}


Next, we need to define the link weight which should satisfies \textbf{(1)} The graph we defined here should be the same with the real state graph. \textbf{(2)} The link weight should reflect the influence strength between those two states. Current works such as gramian based measurement  \cite{conley2000gramian}, empirical definition \cite{sanchez2014hierarchical} are either only applied to linear dynamic system or not the true strength of link weight. In order to get better estimation, we extend the idea of Dynamic structure function \cite{chetty2015network} combining with our Koopman operator. Taking Laplace transform of \ref{eq: 1}, and assuming initial conditions are zeros, yields 
\begin{eqnarray*}
		\left[\begin{matrix}
		sX  \\ s\Psi
	\end{matrix}\right] = \left[\begin{matrix}
		\mathcal{K}_{11} & \mathcal{K}_{12}\\
		\mathcal{K}_{21} & \mathcal{K}_{22}\\
	\end{matrix}\right]	\left[\begin{matrix}
		X  \\ \Psi
	\end{matrix}\right].
\end{eqnarray*}
Solving for $\Psi$  in the second equation and substituting into the first then yields 
\begin{eqnarray}
	sX  = W(s)X \nonumber
\end{eqnarray}
where $W(s) = [\mathcal{K}_{11} + \mathcal{K}_{12}(sI-\mathcal{K}_{22})^{-1}\mathcal{K}_{21}]$. Let $D(s)$ be the matrix of the diagonal entries of $W(s)$, yielding
\begin{eqnarray}
		X = Q(s)X  \label{eq: 2}
\end{eqnarray}
where $Q(s) = (sI-D(s))^{-1}(W(s)-D(s))$. As we can see, $Q(s)$  is a square matrix of strictly proper real rational functions of the Laplace variables with zeros on the diagonal. $Q_{ij}$ would represent the weight  of a directed edge from state $j$ to state $i$; the fact $Q_{ij}$ is proper preserves the meaning of the directed edge as a causal dependency of state $i$ on state $j$. We define the link weight as 
\begin{eqnarray}
	W_{ij} = 
\end{eqnarray} 

==> Section/conclusion.tex <==
\section{conclusion}

==> Section/experiment.tex <==
\section{experiment}

==> Section/reduction.tex <==
\section{Model reduction}

==> Section/system.tex <==
\section{Model Decomposition}
We consider a class of nonlinear systems which have affine control perturbations \textcolor{red}{Cite all of the Isidori and Kotkotovic people}.  Namely we write the system as 
\begin{equation}\label{eq:nonlinear_affine_system}
\begin{aligned}
\dot{x} &= f(x) + g(u)  \\ 
y &= h(x)
\end{aligned}
\end{equation}
where $f,g,h  \in \mathbb{R}^n$ is assumed to be continuously differentiable functions (with $f,g \in C^p\left[0,\infty\right)$ where $p \geq 2$) with respect to $x,u,$ and $t$, respectively.   Without loss of generality, we suppose that $u = 0$ implies that $g(u) = 0$, i.e. any zeroth-order terms in a Taylor expansion of $g(u)$ are subsumed into the definition of $f(x)$. 
\textcolor{red}{Explain for the layman why this is not a loss of generality. Use the Taylor series argument on C-differentiable functions. }

We suppose that $f,g$ and $h$ are time-invariant, i.e. they are directly dependent on $t$.  We model the state $x(t) \in \mathbb{R}^n$ and the input $u(t) \in\mathbb{R}^m$ for all $t \in \left[0,\infty\right).$ 

In this paper, we restrict our attention to nonlinear models that can expressed with an actuated Koopman equation of the form 
\begin{equation}
\dot{\psi}_x(x) = K_x \psi_x(x) + K_u \psi_u(u) 
\end{equation}
    
The Koopman grammian was introduced in \cite{Grammian2017}    
as a way to quantify the controllability and observability of a nonlinear dynamical system.  Here we investigate using the Koopman grammian to obtain a decomposition of the nonlinear system with BIBO stability certificates. 

In our problem, we suppose there are two objectives.  First, we suppose that we want to maximize controllability and observability with respect to a series of input and output channels that represent a system operator's perspective. \textcolor{red}{ Add more writing to clarify what perspectives mean intuitively, motivate blah blah}.  Second, we suppose we want to minimize controllability and observability with respect to a outsider's perspective. 

We model the perturbed system with the form 
\begin{equation}\label{eq:SO_system}
\begin{aligned}
\dot{x} &= f(x) + g(u_S,u_E) \\ &= f(x) + g_S(u_S) + g_E(u_E)  \\ 
y_S &= h_S(x)\\ 
y_E & = h_E(x)  
\end{aligned}
\end{equation}
We suppose, as in \ref{Kutz2015,Williams2016} that an equivalent actuated Koopman system exists for the system (\ref{eq:nonlinear_affine_system}).  
In the presence of two input channels $u_S$ and $u_E$, the question arises as to what the structure of the Koopman system will be.   The following lemma clarifies the system structure. 

\begin{lemma}
Consider system (\ref{eq:nonlinear_affine_system}).  The control Koopman equation for this system is given as 
\begin{equation}
\dot{\psi}(x) = K_x\psi(x)) + K_u\psi_u(u)  
\end{equation}
\end{lemma}
\begin{proof}
More generically, we note that system (\ref{eq:nonlinear_affine_system}), is a special instance of the form of systems studied in \cite{Kutz2015}.  Thus, there exists a control Koopman operator that satisfies the control-Koopman equation
\begin{equation}
\dot{\psi} (x) = K\psi(x,u) 
\end{equation}
Now for our class of nonlinear affine control systems, we know that the Koopman equation can be written \cite{Rowley2015} 
\begin{equation}
\begin{aligned}
\dot{\psi}(x) &= \frac{\partial \psi(x) }{\partial x} \left( f(x) + g(u) \right) \\&=   K\psi(x,u) = K_x \psi_x(x) + K_u \psi_u(u) + K_{xu} \psi_{xu}(x,u)  
\end{aligned}
\end{equation}
where in the last equation we have partitioned $\psi(x,u)$ into terms that directly depend on $x$, $u$, or a mix of the two terms.  Such a partition is always possible, even if one of the terms is trivial.  It suffices to show that the cross-term doesn't exist.  To see this, we take second order partials 

\begin{equation}
\begin{aligned}
 \frac{\partial^2}{\partial u\partial x}\dot{\psi}(x) & =  \frac{\partial^2}{\partial u\partial x} \left(\frac{\partial \psi(x) }{\partial x} \left( f(x) + g(u) \right) \right)\\ &= \frac{\partial^3 \psi(x) }{\partial u \partial^2 x} \left(f(x) + g(u) \right)    \\ & \hspace {3mm} +  \frac{\partial \psi(x) }{\partial x}\frac{\partial}{\partial u}\frac{\partial}{\partial x}\left(f(x) + g(u)\right)\\
 & = 0 
\end{aligned}
\end{equation}
The first term vanishes due to the strict independence of $\psi(x)$ with respect to $u$. 
The second term vanishes due to the affine separation between dependencies of $x$ and $u$ in $f(x)$ and $g(u).$  

In the Koopman equation, taking second order partials results in 
\begin{equation}
\begin{aligned}
\frac{\partial^2}{\partial u\partial x} K\psi(x,u) &=  \frac{\partial^2}{\partial u\partial x} K_x \psi_x(x) + K_u \psi_u(u) + K_{xu} \psi_{xu}(x,u)\\ 
&= 0 + 0 + \frac{\partial^2}{\partial u\partial x} K_{xu} \psi_{xu}(x,u) 
\end{aligned}
\end{equation}
which implies that 
\begin{equation}
\frac{\partial^2}{\partial u\partial x} K_{xu} \psi_{xu}(x,u) = 0 
\end{equation}
By convention, all constant Koopman basis terms are kept in $\psi_x(x)$, which implies that $\psi_{xu}$ has no constant terms, only terms that depend both $x$ and $u$.  The implication of the above equation is that $\psi_{xu}(x,u)$ has only zero and first order terms.  However, since all zero order terms are already in $\psi_x(x)$ and first order terms do not involve mixtures of $x$ and $u$, $\psi_{xu}(x,u) \equiv 0$ for all $x$ and $u.$ 
\end{proof}
This lemma suggests that the system structure of a Koopman operator reflects the dependency structure of the underlying  nonlinear affine system from which it is derived.    In proving this, we have identified a class of nonlinear affine systems that lend themselves to Koopman analysis, and by extension, the classical analysis techniques of control theory for linear time-invariant systems.   However, the Koopman system may be infinite-dimensional.  Whenever the system satisfies Carleman closure \cite{}, then the system is said to have a finite-dimensional Koopman representation.  Otherwise, the  matrices may be infinite-dimensional and require a finite-dimensional approximation. 

We now consider the Koopman system model for a system with external and operator control channels.  The following lemma shows that the structure of the Koopman model mirrors the input structure of system \ref{eq:SO_system}
\begin{lemma}

\end{lemma}


The next lemma is a direct extension of Lemma \ref{lemma:affine_Koopman_partition}

We suppose that an actuated-Koopman equation can be computed for each system model.  We remark that $f(x)$ defines the core dynamics of the system; thus the Koopman operator ${\cal K}_x$ defined with respect to $f$ is the same for both systems, while the Koopman control operator ${\cal K}_u$ and Koopman output equation may be different for each system. 
\begin{lemma}
Given the system (\ref{eq:SO_system}), the Koopman actuated-equations for system operator are of the form 
\begin{equation}
\begin{aligned}
\dot{\psi}^S_x(x) &= K_x^S \psi^S_x(x) + K^S_u \psi^S_u(u) \\
y  &= W^S \psi^S_x(x) 
\end{aligned}
\end{equation}
while the Koopman actuated-equations for the external system (\ref{eq:ES_system}) are given 
\begin{equation}
\begin{aligned}
\dot{\psi}_x^E(x) &= K_x^E \psi^E_x(x) + K^E_u \psi^E_u(u) \\
y  &= W^E \psi^E_x(x) 
\end{aligned}
\end{equation}
Moreover, $\psi^S_x(x) = \psi^S_u(x)$ and $K_x^S = K_x^E.$
\end{lemma}
\begin{proof}
First, from \cite{Kutz2016,Williams2017} \textcolor{red}{Check this reference for rigor!}, we know that a Koopman control equation can be defined for both the external and system model, since they are of the form of $\eqref{eq:nonlinear_affine_system}.$    Moreover, these equations must hold for all $x \in \mathbb{R}^n$ and $u\in\mathbb{R}^m$, including $u=0.$  By construction, $u=0$ implies $\dot{x} = f(x)$ for both systems.   Suppose $\psi^j_u(0) \neq 0$ for $j= S$ or $E$.



Considering the special case $u=0$ which implies $g(u) = 0$, the system then can be regarded as an autonomous system defined by $f(x)$. So for arbitrary $x$, the Koopman actuated equations for system operator and external system should be same. This implies that $K_x^{S} = K_{x}^{E}$.
\end{proof}

\begin{equation}
\begin{aligned}
	\psi_{x}(x_{n}) &= K_x\psi_{x}(x_{n-1}) + K_u\psi_{u}(u_{n-1}) \\
    & = K_{x}^{n}\psi_{x}(x_{0}) + \sum_{i=0}^{n} K_{x}^{i}K_{u}\psi_{u}(u_{i}).
\end{aligned}
\end{equation}
So the lifted Koopman grammian 
\begin{equation}
\begin{aligned}
X_c  &=  \sum_{i=0}^n (K_x)^i K_u K_u^* (K_x^*)^{i} \\
X_o  &= \sum_{i=0}^{n} W(K_x)^{i}(K_x^{*})^{i}W^{*}
\end{aligned}
\end{equation}

Once the models have been cast in the Koopman grammian framework, we can treat the problem as a decomposition on a single dynamical system with two linear time-invariant representations. 

The insider model:
	\begin{eqnarray}
		\dot{x} &=& Ax + B_{in}u, \\
		       y &=& C_{in}x.
	\end{eqnarray}
	And the outsider model:
	\begin{eqnarray}
	\dot{x} &=& Ax + B_{out}u, \\
	y &=& C_{out}x.
	\end{eqnarray}
	
	Generally speaking, $B_{in}, C_{in}$ is much more dense than $B_{out}, C_{out}$. When doing the decomposition for this system, we want to achieve the following property:
	for each subsystem, we want to let the insider have a minimum gramiams, in the meanwhile, outsider have the maximum gramiams. 
	\begin{eqnarray}
		&\min &\sum_{i} \|G_{in}^{i}\| \\
		&\max &\sum_{i} \|G_{out}^{i}\|
	\end{eqnarray}
	To clarify our motivation, let's first consider the following questions:
	\begin{itemize}
		\item (a) We should give the strict definition of insider and outsider ? They are totally different or overlapped ?
		\item (b) We need to give the strict definition of $G_{in}^{i}$ and $G_{out}^{i}$. This relies on clear definition of subsystem(input, output, interconnected factors), then we can compute the gramians .  
		\item (c) What is the incentive for decomposition ? Think about this, 
		assume we don't decompose the system, what should we handle this case ? Another realization ?
		\item (d) If we can do (c), \textcolor{red}{why we do the decomposition}? We should give some motivations here. 
		\item (e) After we have clarified the problems above, the core problem is how to formulate this as an optimization problem even it is NP hard. Always, the clustering problem is NP hard. Our problem is much complicated than normal clustering problem.
        \item (f) If we use Koopman Operator, how could we preserve the structure of our systems ?    
	\end{itemize}
    Also, let's look at the Fig. \ref{fig: motivation}. The left side is our original system. After we do the decomposition, we may find that, for each subsystem, we need to redefine its input, output. \textcolor{red}{So that means our result of partition determines how to compute the gramiams, while in the same time, we also want to do the partition based on gramiams}. This dilemma makes the problem more complicated.  
    \begin{figure}[ht]
    	\centering
    	\includegraphics[width = 8.5cm,height= 4.0cm]{./Figures/motivation}
    	\caption{Model Decomposition}
    	\label{fig: motivation}
    \end{figure}
	To be continued...
	
	
	Some works may be helpful to relief this problem:
	\textcolor{red}{State aggregation} \cite{ishizaki2012clustering} \cite{deng2010building}.  \cite{ishizaki2012clustering} does the  clustering based on the local controlability, however, it has a very strong constraints on the underlying systems. \cite{deng2010building} treats the system a stable Markov process, and does the state aggregation based on minimizing the difference between two Markov process. \\
	
	**********************************************
	\textcolor{red}{The following is our previous idea}.\\
	Consider a continuous time system of the form:
	\begin{eqnarray*}
		\dot{x} &=& f(x)  
	\end{eqnarray*}
    where we assume that $f \in R^{n}$ is continuously differentiable. Our goal is to make a decomposition of  states $X$ such that within each subsystem, the states are strongly infected by each other; in the meanwhile, states outside this subsystem have less influence compared to states within. \textcolor{red}{explanations why we do decomposition}. To do this, we need to solve the following challenges
    \begin{itemize}
    	\item Usually, dynamic system is nonlinear.
    	\item For clustering, how to define the link weight between two states? Also, the graph is directed and contains self-loop links. 
    \end{itemize}

	For the first challenge, our idea here is to use Koopman operator. the Koopman operator is a canonical operator which is the infinite-dimensional map describing the evolution of observables over time. Specially the Koopman operator could be expressed as 
	\begin{eqnarray*}
		\psi(\dot{y}) = \mathcal{K}\psi(y),
	\end{eqnarray*} 
where $\psi(Y)$ is usually an infinite-dimensional observable belong to the subspace of all observables $M_{\psi}$. In this paper, we assume that the original states are contained in these observables. So $Y = [x, \Phi(x)]^{T}$ and we get
	\begin{eqnarray*}
		\psi({[\dot{x}~~\dot{\Phi}(x)]^{T}}) = \mathcal{K}\psi([x~~\Phi(x)]^{T}).
	\end{eqnarray*} 
Also, we use the full state observable $\psi(y = x) = x$ and this will lead to 
\begin{eqnarray}
	\left[\begin{matrix}
		\dot{x}  \\ \dot{\Psi}(x)
	\end{matrix}\right] = \left[\begin{matrix}
		\mathcal{K}_{11} & \mathcal{K}_{12}\\
		\mathcal{K}_{21} & \mathcal{K}_{22}\\
\end{matrix}\right]	\left[\begin{matrix}
     x  \\ \Psi(x)
\end{matrix}\right].  \label{eq: 1}
\end{eqnarray}


Next, we need to define the link weight which should satisfies \textbf{(1)} The graph we defined here should be the same with the real state graph. \textbf{(2)} The link weight should reflect the influence strength between those two states. Current works such as gramian based measurement  \cite{conley2000gramian}, empirical definition \cite{sanchez2014hierarchical} are either only applied to linear dynamic system or not the true strength of link weight. In order to get better estimation, we extend the idea of Dynamic structure function \cite{chetty2015network} combining with our Koopman operator. Taking Laplace transform of \ref{eq: 1}, and assuming initial conditions are zeros, yields 
\begin{eqnarray*}
		\left[\begin{matrix}
		sX  \\ s\Psi
	\end{matrix}\right] = \left[\begin{matrix}
		\mathcal{K}_{11} & \mathcal{K}_{12}\\
		\mathcal{K}_{21} & \mathcal{K}_{22}\\
	\end{matrix}\right]	\left[\begin{matrix}
		X  \\ \Psi
	\end{matrix}\right].
\end{eqnarray*}
Solving for $\Psi$  in the second equation and substituting into the first then yields 
\begin{eqnarray}
	sX  = W(s)X \nonumber
\end{eqnarray}
where $W(s) = [\mathcal{K}_{11} + \mathcal{K}_{12}(sI-\mathcal{K}_{22})^{-1}\mathcal{K}_{21}]$. Let $D(s)$ be the matrix of the diagonal entries of $W(s)$, yielding
\begin{eqnarray}
		X = Q(s)X  \label{eq: 2}
\end{eqnarray}
where $Q(s) = (sI-D(s))^{-1}(W(s)-D(s))$. As we can see, $Q(s)$  is a square matrix of strictly proper real rational functions of the Laplace variables with zeros on the diagonal. $Q_{ij}$ would represent the weight  of a directed edge from state $j$ to state $i$; the fact $Q_{ij}$ is proper preserves the meaning of the directed edge as a causal dependency of state $i$ on state $j$. We define the link weight as 
\begin{eqnarray}
	W_{ij} = 
\end{eqnarray} 
